Guaranteed Privacy-Preserving $\mathcal{H}_{\infty}$-Optimal Interval Observer Design for Bounded-Error LTI Systems

This paper furthers current research into the notion of guaranteed privacy, which provides a deterministic characterization of the privacy of output signals of a dynamical system or mechanism. Unlike stochastic differential privacy, guaranteed privacy offers strict bounds on the proximity between the ranges of two sets of estimated data. Our approach relies on synthesizing an interval observer for a perturbed linear time-invariant (LTI) bounded-error system. The design procedure incorporates a bounded noise perturbation factor computation and observer gains synthesis. Consequently, the observer simultaneously provides guaranteed private and stable interval-valued estimates for a desired variable. We demonstrate the optimality of our design by minimizing the $\mathcal{H}_{\infty}$ norm of the observer error system. Furthermore, we assess the accuracy of our proposed mechanism by quantifying the loss incurred when considering guaranteed privacy specifications. Finally, we illustrate the outperformance of the proposed approach to differential privacy through simulations.

==> macros-abbrev.tex <==
%% Macros for Coordination book
\newcommand{\ds}{\displaystyle}

%%%% enumerate environment containing text and with un-interrupted numbering
\newcounter{saveenum}
%% \setcounter{saveenum}{\value{enumi}}
%% \setcounter{enumi}{\value{saveenum}}

% abbreviations
\newcommand\ie{\mbox{i.e.,\xspace}}
\newcommand\eg{\mbox{e.g.,\xspace}}
\newcommand\etal{\mbox{et~al.,\xspace}}
\newcommand\etc{\mbox{etc.\@\xspace}}
\newcommand\cf{\mbox{cf.\@\xspace}}
\newcommand\resp{\mbox{resp.\@\xspace}}

\newcommand{\e}{\operatorname{e}}

%% Set definitions
\renewcommand{\natural}{{\mathbb{N}}}
\newcommand{\integer}{\ensuremath{\mathbb{Z}}}
\newcommand{\integernonnegative}{\ensuremath{\mathbb{Z}}_{\ge 0}}
\newcommand{\naturalzero}{\integernonnegative} % redundant, to remove
\newcommand{\real}{\ensuremath{\mathbb{R}}}
\newcommand{\realpositive}{\ensuremath{\mathbb{R}}_{>0}}
\newcommand{\realnonnegative}{\ensuremath{\mathbb{R}}_{\ge 0}}
\newcommand{\complex}{\ensuremath{\mathbb{C}}}
\newcommand{\sphere}{\mathbb{S}}
\newcommand{\SO}[1]{\mathrm{SO}(#1)}
\newcommand{\SE}[1]{\mathrm{SE}(#1)}
%% Set operations
\newcommand{\union}{\operatorname{\cup}}
\newcommand{\intersection}{\ensuremath{\operatorname{\cap}}}
\newcommand{\intersect}{\ensuremath{\operatorname{\cap}}}
\newcommand{\bigintersect}{\bigcap}

%% mathematical constructs: \setdef, \until, etc
\newcommand{\until}[1]{\{1,\dots, #1\}}
\newcommand{\subscr}[2]{#1_{\textup{#2}}}
\newcommand{\supscr}[2]{#1^{\textup{#2}}}
\newcommand{\setdef}[2]{\{#1 \; | \; #2\}}
\newcommand{\bigsetdef}[2]{\big\{#1 \; | \; #2\big\}}
\newcommand{\Bigsetdef}[2]{\Big\{#1 \; \big| \; #2\Big\}}
\newcommand{\map}[3]{#1: #2 \rightarrow #3}
\newcommand{\setmap}[3]{#1: #2 \rightrightarrows #3}
\newcommand{\id}{\operatorname{id}}
\newcommand{\diag}[1]{\operatorname{diag}(#1)}
\newcommand{\setofsetvalued}[2]{\mathcal{SC}(#1,#2)}
\newcommand{\spn}{\operatorname{span}}
\newcommand{\image}{\operatorname{image}}

%% mathematical functions
\newcommand{\diam}{\operatorname{diam}}
\newcommand{\radius}{\operatorname{radius}}
\newcommand{\dist}{\operatorname{dist}}
\newcommand{\wdist}{\operatorname{wdist}}
\newcommand{\interior}[1]{\operatorname{int}(#1)}
\newcommand{\oball}[2]{B(#1,#2)}
\newcommand{\bigoball}[2]{B\big(#1,#2\big)}
\newcommand{\Bigoball}[2]{B\Big(#1,#2\Big)}
\newcommand{\cball}[2]{\overline{B}(#1,#2)}
\newcommand{\bigcball}[2]{\overline{B}\big(#1,#2\big)}
\newcommand{\Bigcball}[2]{\overline{B}\Big(#1,#2\Big)}
\newcommand{\der}[2]{\frac{d #1}{d #2}}
\newcommand{\pder}[2]{\frac{\partial #1}{\partial #2}}

%% Symbols from Chp 2 Curves
\newcommand{\signedcurvature}{ \subscr{\kappa}{signed} }
\newcommand{\abscurvature}{ \subscr{\kappa}{abs} }
\newcommand{\radiuscurvature}{\rho}
\newcommand{\normalvector}{\operatorname{n}}
\newcommand{\innormalvector}{\operatorname{n}_{\textup{in}}}
\newcommand{\outnormalvector}{\operatorname{n}_{\textup{out}}}

%% Symbols from Chp 2 Matrix
\newcommand{\identitymatrix}[1]{I_{#1}}
\newcommand{\spectrum}{\operatorname{spec}}
\newcommand{\spectralradius}{\rho}
\newcommand{\essspectralradius}{\subscr{\rho}{ess}}

%% Symbols from Chp 2 Distributed Algorithms
\newcommand{\parts}[1]{\mathbb{P}(#1)}
\newcommand{\finite}[1]{\mathbb{F}(#1)} 
%%% make sure there are no 2^X in the final document
\newcommand{\vect}[1]{\boldsymbol{#1}}
\newcommand{\vectorones}[1][]{\vect{1}_{#1}}
\newcommand{\vectorzeros}[1][]{\vect{0}_{#1}}
\newcommand{\kernel}{\operatorname{kernel}}
\newcommand{\rank}{\operatorname{rank}}
\newcommand{\proj}{\operatorname{proj}}

%% graph
\newcommand{\graph}{G}
\newcommand{\vertices}{V}
\newcommand{\edges}{E}
\newcommand{\adjmat}{A}
\newcommand{\neighbors}{\mathcal{N}}
\newcommand{\neighborsin}{\mathcal{N}^{\textup{in}}}
\newcommand{\neighborsout}{\mathcal{N}^{\textup{out}}}
\newcommand{\length}{\operatorname{length}}
\newcommand{\weight}{\operatorname{weight}}
\newcommand{\reverse}{\operatorname{rev}}
\newcommand{\TBFS}{\ensuremath{\subscr{T}{BFS}}\xspace}
\newcommand{\TDFS}{\ensuremath{\subscr{T}{DFS}}\xspace}
\newcommand{\Tshpt}{\ensuremath{\subscr{T}{shortest-paths}}\xspace}
%% \newcommand{\TMST}{\ensuremath{\subscr{T}{MST}}\xspace}
%% \newcommand{\TSP}{\ensuremath{\subscr{T}{TSP}}\xspace}
\newcommand{\algofont}[1]{\textsc{#1}}
\newcommand{\algostep}[1]{{\small\texttt{#1:}}\xspace}

%% Chp2: state machines and dynamical systems
\newcommand{\equilibria}[1]{\operatorname{Equil}(#1)}
\newcommand{\lieder}[2]{\mathcal{L}_{#1}#2}

%% Chp2: synchronous network
\newcommand{\network}[1][]{\mathcal{S}_{\textup{#1}}}
\newcommand{\Ecmm}{\subscr{E}{cmm}}

\newcommand{\alphabet}{\mathbb{A}}

%% robot and environment sensing: function, alphabet, symbol
\newcommand{\rbtsns}{\textup{rbt-sns}\xspace}
\newcommand{\rbtalphabet}{\subscr{\mathbb{A}}{rbt}}
\newcommand{\rbts}{y}

\newcommand{\envsns}{\textup{env-sns}\xspace}
\newcommand{\envalphabet}{\subscr{\mathbb{A}}{env}}
\newcommand{\envs}{\subscr{y}{env}}


\newcommand{\supind}[2]{{#1}^{[#2]}}
\newcommand{\superscr}[2]{{#1}^{\operatorname{#2}}}
\newcommand{\subind}[2]{{#1}_{[#2]}}
\newcommand{\DA}[1][]{\mathcal{D\!A}_{\textup{#1}}}
\newcommand{\timeschedule}{\integernonnegative}
\newcommand{\edtimeschedule}{\Sigma}
\newcommand{\nll}{\mytt{null}}
\newcommand{\msg}{\textup{msg}\xspace}
\newcommand{\stf}{\textup{stf}\xspace}
\newcommand{\msgig}{\textup{msg-trig}\xspace}
\newcommand{\stftrig}{\textup{stf-trig}\xspace}
\newcommand{\msggen}{\textup{msg-gen}\xspace}
\newcommand{\msgrec}{\textup{msg-rec}\xspace}
\newcommand{\msgstandard}{\textup{msg}_{\textup{std}}}
\newcommand{\TC}{\operatorname{TC}}
\newcommand{\SC}{\operatorname{SC}}
\newcommand{\CC}{\operatorname{CC}}

%% algorithmic enviroment fixes
\newcommand{\AND}{AND\xspace}
\newcommand{\OR}{OR\xspace}
\newcommand{\return}{\textbf{return}\xspace}
\newcommand{\mycase}{\textbf{case}\xspace}
\newcommand{\mytt}[1]{\textup{\texttt{#1}}\xspace} %% mytt = my typefont text
\newcommand{\true}{\mytt{true}}
\newcommand{\false}{\mytt{false}}
\newcommand{\data}{\mytt{data}}
\newcommand{\newdata}{\mytt{new-data}}
\newcommand{\leader}{\mytt{leader}}
\newcommand{\newleader}{\mytt{new-lead}}
\newcommand{\transmit}{\mytt{transmit}}
\newcommand{\newtransmit}{\mytt{new-transmit}}
\renewcommand{\transmit}{\mytt{snd-flag}}
\renewcommand{\newtransmit}{\mytt{new-snd-flag}}
\newcommand{\search}{\mytt{search}}
\newcommand{\newsearch}{\mytt{new-search}}
\newcommand{\round}{\mytt{round}}
\newcommand{\unknown}{\mytt{unknwn}}
\newcommand{\maxuid}{\mytt{max-id}}
\newcommand{\newuid}{\mytt{new-id}} 
\newcommand{\uid}{\mytt{uid}}
\newcommand{\uuu}{\mytt{my-id}}
\newcommand{\parent}{\mytt{parent}}
\newcommand{\newparent}{\mytt{new-parent}}
\newcommand{\mydist}{\mytt{dist}}
\newcommand{\newdist}{\mytt{new-dist}}
\newcommand{\mypar}{\mytt{parent}}

%% Chp2: linear iterations
\newcommand{\TwoNorm}[1]{\|#1\|_2}
\newcommand{\bigTwoNorm}[1]{\big \|#1 \big \|_2}
\newcommand{\BigTwoNorm}[1]{\Big \|#1 \Big \|_2}
\newcommand{\PNorm}[1]{\|#1\|_p}
\newcommand{\InftyNorm}[1]{\|#1\|_{\infty}}
\newcommand{\ymaxmin}{\subscr{y}{max-min}}
\newcommand{\yerr}{\subscr{y}{err}}
\newcommand{\expfac}{\subscr{r}{exp}}

\newcommand{\tridmat}{\operatorname{Trid}}
\newcommand{\atridmat}{\operatorname{ATrid}}
\newcommand{\circmat}{\operatorname{Circ}}
\newcommand{\yave}{\subscr{y}{ave}}
\newcommand{\xave}{\subscr{x}{ave}}
\newcommand{\zave}{\subscr{z}{ave}}

\newcommand{\complexnorm}[1]{\|#1\|_\complex}
\newcommand{\Bigcomplexnorm}[1]{\Big\|#1\Big\|_\complex}
\newcommand{\norm}[2]{\|#1\|_{#2}}
\newcommand{\bignorm}[2]{\big\|#1\big\|_{#2}}
\newcommand{\Bignorm}[2]{\Big\|#1\Big\|_{#2}}
\newcommand{\Biggnorm}[2]{\Bigg\|#1\Bigg\|_{#2}}
\newcommand{\Enorm}[1]{\|#1\|_{2}}

\newcommand{\ii}{i_{\mathbb{F}}}

%% proof of number theory result
\newcommand{\mquot}{\subscr{m}{qtnt}}
\newcommand{\mremain}{\subscr{m}{rmndr}}



%% Set of matrices
\newcommand{\stoch}[1]{{\cal F}(#1)}
\newcommand{\substoch}[2]{{\cal F}_{#2}(#1)}

%% Symbols from Chp 3 Geometry
\newcommand{\PP}{\mathcal{P}}
\newcommand{\eps}{\varepsilon}
\renewcommand{\epsilon}{\varepsilon}
\newcommand{\ov}{\overline}
\newcommand{\fti}{\operatorname{fti}}
\newcommand{\visibilityset}[2]{\operatorname{Vi}(#1;#2)}
%% \newcommand{\robustvisibilityset}[3]{\operatorname{Vi}_{#3}(#1;#2)}

%% range-limited visibility set; defined chapter 4 or 5
\newcommand{\rlvs}[2]{\subscr{\operatorname{Vi}}{disk}(#1;#2)}


%% distances
\newcommand{\distC}{\operatorname{\subscr{dist}{\texttt{c}}}}
\newcommand{\distCC}{\operatorname{\subscr{dist}{\texttt{cc}}}}

%% polytopes
\newcommand{\chull}[1]{\operatorname{co}(#1)}
\newcommand{\rchull}[2]{\operatorname{rco}_{#2}(#1)}
\renewcommand{\rchull}[2]{\operatorname{rco}(#1;#2)}
\newcommand{\co}{\operatorname{co}}

%% geometric centers
\newcommand{\ccenter}[1]{\operatorname{CC}(#1)}
\newcommand{\ccenterBig}[1]{\operatorname{CC}\!\big(#1\big)}
\newcommand{\icenter}[1]{\operatorname{IC}(#1)}
\newcommand{\cradius}[1]{\operatorname{CR}(#1)}
\newcommand{\iradius}[1]{\operatorname{IR}(#1)}
\newcommand{\area}[2]{\operatorname{A}_{#2}(#1)}
\newcommand{\centroid}[2]{\operatorname{CM}_{#2}(#1)}
\newcommand{\momentofinertia}[3]{\operatorname{J}_{#2}(#1,#3)}
\newcommand{\verticespolytope}[1]{\operatorname{Ve}(#1)}
\newcommand{\facetspolytope}[1]{\operatorname{Fa}(#1)}
\newcommand{\edgespolytope}[1]{\operatorname{Ed}(#1)}
\newcommand{\density}{\phi}
\newcommand{\Voronoi}[1]{\mathcal{V}(#1)}
\newcommand{\limVoronoi}[1]{\mathcal{V}_r(#1)}

%% proximity graphs
\newcommand{\proximitygraph}{\mathcal{G}} 
\newcommand{\edgesproximitygraph}[1]{\mathcal{E}_{#1}} 
\newcommand{\neighborsproximitygraph}{\mathcal{N}}
\newcommand{\completegraph}{\subscr{\proximitygraph}{cmplt}}
\newcommand{\rdiskgraph}{\subscr{\proximitygraph}{disk}(r)}
\newcommand{\ridiskgraph}{\subscr{\proximitygraph}{$\infty$-disk}(r)}
\newcommand{\Dgraph}{\subscr{\proximitygraph}{D}}
\newcommand{\rDgraph}[1]{\subscr{\proximitygraph}{LD}(#1)}
\newcommand{\aDgraph}{\subscr{\proximitygraph}{LD}(a)}
\newcommand{\RNgraph}{\subscr{\proximitygraph}{RN}}
\newcommand{\Ggraph}{\subscr{\proximitygraph}{G}}
\newcommand{\EMSTgraph}{\subscr{\proximitygraph}{EMST}}
\newcommand{\EMSTGgraph}[1]{\subscr{\proximitygraph}{EMST,$#1$}}
\newcommand{\Vgraph}[1]{\subscr{\proximitygraph}{vis,$#1$}}
\newcommand{\Vdiskgraph}[1]{\subscr{\proximitygraph}{vis-disk,$#1$}}
\newcommand{\ClessVdiskgraph}[1]{\subscr{\proximitygraph}{lc-vis-disk,$#1$}}
%% \newcommand{\RVgraph}{\subscr{\proximitygraph}{$\eps$-vis,Q}}
\newcommand{\LCgraph}[1]{\subscr{\proximitygraph}{lc,$#1$}}

\newcommand{\osegment}[2]{]#1,#2[}
\newcommand{\csegment}[2]{[#1,#2]}
\newcommand{\ocsegment}[2]{]#1,#2]}

%% geometric optimization
\newcommand{\HH}{\mathcal{H}}
\newcommand{\HHexp}{\mathcal{H}_{\textup{exp}}}
\newcommand{\HHdistor}{\mathcal{H}_{\textup{dist}}}
\newcommand{\HHarea}[1]{\mathcal{H}_{\textup{area},#1}}
\newcommand{\HHmixed}[1]{\mathcal{H}_{\textup{dist-area},#1}}
\newcommand{\HHworst}{\mathcal{H}_{\textup{worst}}}
\newcommand{\HHdc}{\mathcal{H}_{\textup{dc}}}
\newcommand{\HHsp}{\mathcal{H}_{\textup{sp}}}
\newcommand{\HHsum}{\mathcal{H}_\Sigma}
\newcommand{\HHmax}{\mathcal{H}_{\max}}
\newcommand{\performance}{f}
\newcommand{\coincident}{\mathcal{S}_{\textup{coinc}}}
\newcommand{\indicator}[1]{\operatorname{1}_{#1}}
\newcommand{\arc}{\operatorname{arc}}
\newcommand{\discont}[1]{\operatorname{Dscn}(#1)}

%% maybe to move into Chap 2
\newcommand{\scalarproduct}[2]{#1 \cdot #2}

%% Symbols from Chp 4 Model
\newcommand{\groupop}{\star}
\newcommand{\groupidentity}{e}
\newcommand{\so}{\mathfrak{so}}

%% Feedback communication and control + Tasks
\newcommand{\setofrobots}{\mathcal{R}}
\newcommand{\robot}{R}
\newcommand{\ctrl}{\textup{ctl}}
\newcommand{\received}[1]{\subscr{#1}{rcvd}}
\newcommand{\sensed}[1]{\subscr{#1}{snsd}}
\newcommand{\sampled}[1]{\subscr{#1}{smpld}}
\newcommand{\FCC}[1][]{\mathcal{CC}_{\textup{#1}}}
\newcommand{\ECC}[1][]{\mathcal{ECC}_{\textup{#1}}}
\newcommand{\SFC}[1][]{\mathcal{RSC}_{\textup{#1}}}
\newcommand{\task}[1][]{\mathcal{T}_{\textup{#1}}}

%% Systems Names -- polish following names: why are there 2 for each shit?
\newcommand{\disk}{disk}
\newcommand{\rdisk}{\textup{disk}}
\newcommand{\circledisk}{circle}
\newcommand{\umax}{\subscr{u}{max}}
\newcommand{\rIdisk}{$\infty$-disk}
\newcommand{\LD}{\textup{LD}}
\newcommand{\visdisk}{vis-disk}

\newcommand{\rs}[1]{\supscr{#1}{rs}}

%% FCC Names
\newcommand{\agreepursueName}{\algofont{agree \& pursue}\xspace}
\newcommand{\agreepursue}{\algofont{agree \& pursue}} %% why two?
\newcommand{\agreepursueModName}{\algofont{mod-agree \& pursue}\xspace}

\newcommand{\VicsekName}{\algofont{averaging}\xspace}
\newcommand{\circumcenter}{\algofont{crcmcntr}\xspace}
\newcommand{\nonconvexcircumcenter}{\algofont{nonconvex crcmcntr}\xspace}
\newcommand{\sensorcircumcenter}{\algofont{relative-sensing crcmcntr}\xspace}
\newcommand{\nonconvexsensorcircumcenter}{\algofont{nonconvex relative-sensing crcmcntr}\xspace}

\newcommand{\parallelcircumcenter}{\algofont{pll-crcmcntr}\xspace}
\newcommand{\parallelccenter}[1]{\operatorname{PCC}(#1)}

\newcommand{\VoronoiCentroid}{\algofont{Vrn-cntrd}\xspace}
\newcommand{\VoronoiCentroidDynamics}{\algofont{Vrn-cntrd-dynmcs}\xspace}
\newcommand{\LimitedVoronoiNormal}{\algofont{Lmtd-Vrn-nrml}\xspace}
\newcommand{\LimitedVoronoiCentroid}{\algofont{Lmtd-Vrn-cntrd}\xspace}
\newcommand{\sensorLimitedVoronoiCentroid}{\algofont{relative-sensing Lmtd-Vrn-cntrd}\xspace}
\newcommand{\RangeVoronoiCentroid}{\algofont{Rng-Vrn-cntrd}\xspace}
\newcommand{\VoronoiCircumcenter}{\algofont{Vrn-crcmcntr}\xspace}
\newcommand{\VoronoiIncenter}{\algofont{Vrn-ncntr}\xspace}

%% Task Names
\newcommand{\equidistance}{eqdstnc}

%% Sensor-based networks
\newcommand{\wrt}[2]{ \subscr{#1}{#2} }
\newcommand{\what}[2]{ \supscr{#1}{#2} }

%% Costs
\newcommand{\MCC}{\operatorname{MCC}}
\newcommand{\TCC}{\operatorname{TCC}}
\newcommand{\cc}{\operatorname{IH-MCC}}
\newcommand{\unidir}{\operatorname{unidir}}
\newcommand{\omnidir}{\operatorname{omnidir}}
\newcommand{\nonnllmsgs}{{cmm$\setminus\emptyset$}}
\newcommand{\CommCost}[1][]{\subscr{\operatorname{C}}{rnd}^{#1}}


%%% more about the agree and pursue
\newcommand{\dm}{\mytt{dir}}
\newcommand{\newdm}{\mytt{new-dir}}
\newcommand{\csym}{\mytt{c}}
\newcommand{\ccsym}{\mytt{cc}}
\newcommand{\kprop}{\subscr{k}{prop}}
\newcommand{\Hset}{H}%
\newcommand{\nHset}{n_H}%

%%% random definitions
\newcommand{\fl}[1]{\left\lfloor #1\right\rfloor}
\newcommand{\argmin}{\ensuremath{\operatorname{argmin}}}
\newcommand{\argmax}{\ensuremath{\operatorname{argmax}}}
\newcommand{\arginf}{\ensuremath{\operatorname{arginf}}}
\newcommand{\argsup}{\ensuremath{\operatorname{argsup}}}
\newcommand{\myboolean}{\ensuremath{\{\true,\false\}}} %%to erase

\newcommand{\WW}{{\mathcal{W}}}
\newcommand{\MM}{\mathcal{M}}
\newcommand{\Pc}{{\mathcal{P}}}
\newcommand{\reschedule}[3]{{#1}_{(#2,#3)}}
\newcommand{\newC}{\CommCost[]\circ\MM}
\newcommand{\Infnorm}[1]{\|#1\|_{\infty}}

%% symbols for Chp5: rendezvous

%% connectivity maintenance
\newcommand{\XConstrSet}{\mathcal{X}}
\newcommand{\XConstrSetVis}{\subscr{\mathcal{X}}{\visdisk}}
\newcommand{\XConstrSetClessVis}{\subscr{\mathcal{X}}{lc-\visdisk}}

%%\newcommand{\Dc}{\subscr{\UConstrSet}{constraint}}
%%\newcommand{\UConstrSet}{\mathcal{U}}
%%\newcommand{\UConstrSetVis}{\subscr{\mathcal{U}}{\visdisk}}

\newcommand{\rendezvous}{rndzvs}
\newcommand{\ccsalgo}{\algofont{iterated truncation}\xspace}
\newcommand{\rsccsalgo}{\algofont{relative-sensing iterated truncation}\xspace}
\newcommand{\average}{\operatorname{avrg}}
\newcommand{\vers}{\operatorname{vers}}
\newcommand{\piSpace}[1]{\pi_{#1}}


\newcommand{\maximize}{\text{maximize}}
\newcommand{\subj}{\text{subject to}}

\newcommand{\mynum}[1]{{\small\ensuremath{{\texttt{#1}}}\xspace}}

\newcommand{\EE}{\mathcal{E}}
\newcommand{\NN}{\mathcal{N}}
\newcommand{\FF}{\mathcal{F}}

%% copyright
\newcommand\reg{$^{\textrm{\tiny\textregistered}}$\xspace}

%% packages for Chp5

\usepackage{psfrag}

%% symbols for Chp 6: Deployment

\newcommand{\deployment}{dply}
\newcommand{\deploymentdistor}{distor-\deployment}
\newcommand{\deploymentarea}{area-\deployment}
\newcommand{\deploymentmixed}{distor-area-\deployment}
\newcommand{\deploymentdc}{dc-\deployment}
\newcommand{\deploymentdcwk}{dc-wk-deployment}
\newcommand{\deploymentsp}{sp-\deployment}
\newcommand{\deploymentspwk}{sp-wk-deployment}

\newcommand{\fcase}[1]{\ensuremath{(\mathbf{#1})}\xspace}
\newcommand{\Pave}{\subscr{P}{ave}}

\newcommand{\centrd}{centrd}
\newcommand{\XX}{\mathcal{X}}
\newcommand{\incenVor}{incntr-Vor}
\newcommand{\circumVor}{crcntr- Vor}

%% symbols for Chp 7: estimation
\newcommand{\Kstf}[1]{\subscr{\supind{K}{#1}}{stf}}
\newcommand{\Kstfna}{\subscr{K}{stf}}

\newcommand{\nip}{\subscr{n}{ip}}
\newcommand{\pdistance}{\mathcal{D}_\lambda}
\newcommand{\arclengthdist}{\subscr{\mathcal{D}}{arc}}
\newcommand{\kapadistance}{\subscr{\mathcal{D}}{curvature}}

\newcommand{\nw}{\mytt{nxt}}
\newcommand{\nwrec}{\mytt{nxtrec}}
\newcommand{\curves}{\mathcal{C}}
\newcommand{\mypath}{\mytt{path}}
\newcommand{\tpath}{\mytt{t}_\mytt{path}}
\newcommand{\tangentat}{\mytt{tangentat}}
\newcommand{\cyclicbalance}{\mytt{cyclic-balance}}
\newcommand{\perpproj}{\mytt{perp-proj}}
\newcommand{\sat}{\operatorname{sat}}
\newcommand{\inclusion}{\operatorname{\iota}}

\newcommand{\eul}{\textsc{Single-Robot Estimate Update Law}\xspace}
\newcommand{\ceul}{\textsc{Cooperative Estimate Update Law}\xspace}
\newcommand{\eupl}{\textsc{Estimate Update and Balancing Law}\xspace}
\newcommand{\aupl}{\textsc{Approximate Estimate and Balancing Law}\xspace}

%% %% OLD ??
%% \newcommand{\optplace}{\mytt{opt-place}}

%% \newcommand{\lw}{\mytt{L}}
%% \newcommand{\setpath}{\operatorname{path}}
%% \newcommand{\regionest}{\mytt{\polygon}}

%% \newcommand{\timewindow}{\mytt{t}}
%% \newcommand{\prev}{\mytt{qprev}}
%% \newcommand{\apdistance}{\mytt{d}}


%% \newcommand{\forget}{\mytt{forget}}

\newcommand{\arclengthparam}{\subscr{s}{arc}}
\newcommand{\gammaarc}{\subscr{\gamma}{arc}}
% \newcommand{\arclength}{\subscr{\gamma}{arc}}
\newcommand{\gammapolar}{\subscr{\gamma}{polar}}
\newcommand{\sign}{\operatorname{sign}}

\newcommand{\Vc}{{\mathscr{V}}}
\newcommand{\Wc}{{\mathscr{W}}}
\newcommand{\Tc}{{\mathscr{T}}}
\newcommand{\Cc}{{\mathscr{C}}}
\newcommand{\Ec}{{\mathscr{E}}}
\newcommand{\DD}{{\mathcal{D}}}
\newcommand{\UU}{{\mathcal{U}}}
\newcommand{\LL}{{\mathcal{L}}}
\newcommand{\ip}{{\mytt{q}}}
\newcommand{\SeqNorm}[1]{\|#1\|_{2,\infty}}
\newcommand{\classK}{\ensuremath{\mathcal{K}}}
\newcommand{\classKinfty}{\ensuremath{\mathcal{K}_{\infty}}}
\newcommand{\classKL}{\ensuremath{\mathcal{KL}}}
\newcommand{\NearNeigh}{\text{NN}}
\newcommand{\NatNeigh}{\text{Nat}}
\newcommand{\triangular}{\text{TIN}}
\newcommand{\inverse}{\text{IDW}}
\newcommand{\localinv}{\text{LIDW}}
\newcommand{\QQ}{\mathcal{Q}}
\newcommand{\MSE}{\operatorname{MSE}}

\newcommand{\Tmin}{\subscr{T}{min}}
\newcommand{\ymin}{\subscr{y}{min}}
\newcommand{\xfree}{\supscr{x}{free}}
\newcommand{\xctrl}{\supscr{x}{ctrl}}

%\renewcommand{\ymaxmin}{\subscr{y}{M-m}}
\newcommand{\Aerr}{\subscr{F}{err}}
\newcommand{\cerr}{\subscr{c}{err}}
\newcommand{\Derr}{\subscr{D}{err}}
\newcommand{\Dave}{\subscr{D}{ave}}
\newcommand{\yerrtilde}{\subscr{\tilde{y}}{err}}

\setlength{\tabcolsep}{3pt}

